Certified Patch Robustness via Smoothed Vision Transformers

Certified patch defenses can guarantee robustness of an image classifier to arbitrary changes within a bounded contiguous region. But, currently, this robustness comes at a cost of degraded standard accuracies and slower inference times. We demonstrate how using vision transformers enables significantly better certified patch robustness that is also more computationally efficient and does not incur a substantial drop in standard accuracy. These improvements stem from the inherent ability of the vision transformer to gracefully handle largely masked images. Our code is available at https://github.com/MadryLab/smoothed-vit.

==> sections/app-pretrained.tex <==

\subsection*{Ablation Accuracy}
\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/pretrained/cifar10_ablation_acc.pdf}
        \caption{Pretrained CIFAR-10 models.}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pretrained/ImageNet_ablation_acc.pdf}
        \caption{Pretrained ImageNet models.}
    \end{subfigure}
\caption{Ablation accuracies for pretrained models on CIFAR-10 and ImageNet column-ablated images. ViTs outperforms ResNets by a significant margin, especially on ImageNet.}
\label{fig:pretrained}
\end{figure}
Without training on image ablations, we find that pretrained ViTs naturally maintain significantly higher accuracy on column ablations than comparably sized ResNets as shown in Figure \ref{fig:pretrained}. 
This difference is most prominent on ImageNet---ViT-B has 30-40\% higher ablation accuracy across a range of ablation sizes than the largest residual network (WRN-101-2), which suggests that ViTs are naturally better suited for classifying image ablations. 
Even when models are fine-tuned for image ablations, we find that a significant gap still remains. 
For example, the ViT-S has 11-12\% higher ablation accuracy than the ResNet-50 over the same ablation sizes. 

\subsection*{Certified Accuracy}
\paragraph{Pretrained vision transformers are certifiably robust}
\label{sec:pretrained}

In this subsection, we test how certifiably robust are of-the-shelf pretrained ViTs and ResNets when smoothed with derandomized smoothing. Recall that pretraind ViTs are able to classify small ablations of images much better than ResNets as we showed in Section~\ref{sec:ablations} and Figure~\ref{fig:pretrained} for various ablation sizes. This suggests that is we apply derandomized smoothing on ViTs, they will outperform ResNets. We apply derandomized smoothing, as described in Section~\ref{sec:background-derandomized}. We use column smoothing with ablation sizes of $s = 19$ and $s=XX$ on ImageNet and CIFAR-10, respectively. We sweep over the various ViTs and ResNets listed in see Section~\ref{sec:why}. ViTs consistently achieve substantially higher certificates of robustness than ResNets across all architecture as shown in Figure~TODO againts various sizes of adversarial patches. For example ViT-B achieves around $32\%$ certified accuracy on  ImageNet against $42 \times 42$ adversarial patches, whereas a larger-size WRN-101-2 achieves only $2\%$.

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{.48\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/pretrained/cifar10_cert_acc.pdf}
        \caption{Pretrained CIFAR-10 models.}
    \end{subfigure}
    \begin{subfigure}[b]{.48\textwidth}
        \centering
            \includegraphics[width=\textwidth]{figures/pretrained/imagenet_cert_acc.pdf}
            \caption{Pretrained ImageNet models.}
        \end{subfigure}
    \caption{Certified accuracy of various \textbf{pretrained} ViTs and comparable size ResNets on CIFAR-10 and ImageNet. ViTs non-trivial robustness wheras ResNets do not.}
    \label{fig:pretrained-certified-vary-s}
\end{figure}


==> sections/checklist.tex <==
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See the conclusion.}
    % \answerYes{See Section~\ref{sec:conclusions}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See the conclusion.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  \answerYes{The code link is in the abstract.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Appendix.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite both ImageNet and CIFAR-10 in the main paper.}
  \item Did you mention the license of the assets?
    \answerYes{See Appendix.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
    \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/improvements.tex <==
In the previous section, we showed that Vision Transformers can maintain higher accuracy than ResNets when classifying image ablations and can speed up the runtime of evaluating masked images. Both of these properties strongly suggest that Vision Transformers are highly suitable for de-randomized smoothing.

%In this section, we evaluate the performance of de-randomized smoothing using ResNets and Vision Transformers for the base model. 
In this section, we find that using Vision Transformers substantially improves multiple metrics for de-randomized smoothing. 
First, we see substantial gains in certified accuracy of de-randomized smoothing over using comparably sized ResNets. 
Second, smoothed transformers maintain standard accuracy competitive with standard models, unlike smoothed ResNets. %rendering them more practical for real applications. 
%Finally, we evaluate the computation speed of certifying with ResNets versus transformers 
Third, vision transformers have significantly reduced the runtime for both training and evaluation with the dropped token optimization from Section \ref{sec:why}. 

Here, we focus primarily on the column smoothing setting and defer block smoothing results to Appendix \ref{app:block-smoothing}. Our experimental setup is the same as the previous Section \ref{sec:why} and is similar to \citet{levine2020randomized}. 


% \eric{Need to reference block smoothing in appendix.}

\begin{figure}[!htbp]
    \centering
    \includegraphics[trim=0 0 140 0, clip, width=.375\textwidth]{figures/finetuned_vs_patchsize/cifar10_cert_acc.pdf}
    \includegraphics[width=.5\textwidth]{figures/finetuned_vs_patchsize/imagenet_cert_acc.pdf}  
\caption{Certified accuracies for ViT and ResNet models on CIFAR-10 and ImageNet for various adversarial patch sizes. Certification was performed using a fixed alation size $b=4$ for CIFAR-10 and $b=19$ for ImageNet following \cite{levine2020randomized}.\ericinline{Group legend by size, not architecture?}}
\label{fig:certified-vs-patchsize}
\end{figure}

\begin{table}
    \caption{Standard accuracies for smoothed ViTs and ResNets on CIFAR-10 and ImageNet. Certification was performed was performed using a fixed alation size $b=4$ for CIFAR-10 and $b=19$ for ImageNet. 
    \ericinline{delineate with horizontal rules instead of vertical}}
    \centering
    \begin{tabular}{lcc|cc|cc}
        \toprule
        {} & \multicolumn{6}{c}{Standard Accuracy of Smoothed Classifier (\%)} \\
        Architecture &             ViT-T &   ResNet-18 & ViT-S &  ResNet-50 & ViT-B & WRN-101 \\
        \midrule
        ImageNet &            \textbf{52.25} &  50.62 &    \textbf{63.48} &  51.47 &   \textbf{69.33} &     61.38 \\
        CIFAR-10 &            \textbf{86.03} &  84.75 &    \textbf{89.36} &  87.42 &   \textbf{91.73} &     89.10 \\
                \bottomrule
    \end{tabular}
    \label{table:standard-smoothed-acc}
\end{table}


\paragraph{Certified patch robustness}
%We evaluate the certification guarantees for column-smoothed ViTs and ResNets. 
%As in \cite{levine2020randomized}, we perform smoothing with a fixed ablation size of $b=19$ for ImageNet and $b=4$ for CIFAR-10, and evaluate the certified accuracy of the models over a range of adversarial patch sizes (Figure \ref{fig:certified-vs-patchsize}). 
We find that using vision transformers for the base classifier boosts certified accuracy over ResNets across a range of model sizes. 
For example, against $32\times 32$ adversarial patches on ImageNet (2\% of the image), a smoothed ViT-S improves certified accuracy by 14\% over a smoothed ResNet50,\footnote{We found that ResNets could achieve a significantly higher certified accuracy than was reported by \citep{levine2020randomized} when using early stopping-based model selection, which we elaborate on in Appendix \ref{app:setup}} while the larger ViT-B reaches a certified accuracy of 39\%---well above the highest reported baseline of 28\% \citep{}.\footnote{The highest reported certified accuracy in the literature for this patch size on ImageNet is 28\% from Patchguard \citep{xiang2021patchguard}. However, this defense uses a masking technique that is optimized for this particular patch size, and achieves 0\% certified accuracy against patch larger than $32\times 32$.}
\eric{Need to include the baselines in either a table or a figure}


\paragraph{Smoothed accuracy}
% \eric{We should shorten this, i.e. instead of repeating numbers that are in the figures, we can just say what the improvement is.}
A significant challenge for certified robustness in general is the precipitous drop in standard accuracy. 
De-randomized smoothing is no exception: a smoothed ResNet-50 drops over 27\% in standard accuracy over a regular ResNet-50. 
We find that \svit{} do not suffer from as dramatic of a degradation: for example, the smoothed ViT-B has a standard accuracy of 69\%, which is 13\% lower than a standard ViT-B. 
In section \ref{sec:probe}, we show how the standard accuracy can improve even further---by more than 4\% on ImageNet---without sacrificing certified performance. 
%smoothing a VIT-S, for example, leads to a clean accuracy of 63.48\%, which is only \saachiinline{X}\% lower than a standardly trained VIT-S. By maintaining a competitively high clean accuracy, \svit{} can provide strong guarantees without a serious drop in performance. \saachi{do we want to put what the standard accuracy of the non-smoothed models in the table?}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/scalability/scalability_eval.pdf}
        \caption{Evaluation speed (forward pass)}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/scalability/scalability_train.pdf}
        \caption{Training speed (forward and backward pass)}
    \end{subfigure}
\caption{(a) Average speed (over 50 trials) of computing a forward pass on a batch of 1024 image ablations on ImageNet (b) Average speed (over 50 trials) of computing a full training step (forward and backward pass) on a batch of 128 image ablations on ImageNet}
\label{fig:scalability}
\end{figure}

\begin{table}
    \begin{center}
    \caption{Multiplicative speed up of using a vision transformer with dropped tokens over a ResNet, measured for a forward pass of 1024 column ablated ImageNet images with column size $b=19/224$ averaged over 50 trials.}
    % \caption{We measure the average speed (over 50 trials) of computing a forward pass on 1024 column ablated images with ablation size $b=19$. We report the multiplicative speed up of using a vision transformer (dropping masked tokens) over a ResNet).}
    \label{tab:speed_resnet}
    \begin{tabular}{c|ccc}
    \toprule
    & ResNet-18 & ResNet-50 & WRN-101\\
    \midrule
    ViT-T & \textbf{5.85x} & 21.96x & 101.99x \\
    ViT-S & 2.85x & \textbf{10.68x} & 49.62x \\
    ViT-B & 1.26x & 4.75x & \textbf{22.04x} \\
    \bottomrule
    \end{tabular}
    \end{center}
\end{table}

\paragraph{Faster Certification} 
Another drawback of de-randomized smoothing is its high computational cost: the base classifier must classify all image ablations before making a prediction (and certification). 
We find that this computational cost is significantly alleviated when dropping masked tokens as described in Section \ref{sec:why}. 

In Figure \ref{fig:scalability} we measure the speed of processing a batch of image ablations in both training (forward and backward) and evaluation (only forward) settings across multiple ablation sizes. 
We find that ViTs that drop tokens are vastly faster than similarly sized ResNets. 
For example, using a ViT-S (when dropping fully masked tokens) gives an average speed up of 10.68x over a ResNet-50 when evaluating column ablated images with an ablation size $b=19$ (Table \ref{tab:speed_resnet}).
In fact, even the largest ViT-B architecture is 1.25x faster than a ResNet-18, despite being TODOx larger in parameter count. 
\eric{We should include an architecture size table in the appendix}
\saachi{should we say gpu specs here? this was on an a100}
%In Section \ref{sec:why}, we found that dropping masked tokens when using a transformer can significantly improve efficiency. In Figure \ref{fig:scalability}, we examine the speed of computing over a batch of image ablations in both a training (forward and backward) and evaluation (only forward) setting across multiple ablation sizes. We find that using transformers with this optimization significantly speeds up certification in comparison to similarly sized ResNets. For example, using a VIT-S (when dropping fully masked tokens) gives an average speed up of 10.68x over a ResNet-50 when evaluating column ablated images with an ablation size $b=19$ (Table \ref{tab:speed_resnet}).\saachi{should we say gpu specs here? this was on an a100}
% \eric{Yes we need specs.}

==> sections/probing.tex <==
% IGNORE THIS FILE
% At the core of any smoothed model is the set of image ablations used to smooth the model. 
% However, specific choices in image ablation such as the type, amount, and size can significantly affect trade-offs between certified robustness and other metrics such as clean accuracy and inference speed. 
% In this section, we demonstrate how these choices affect the smoothed model and the corresponding trade-offs through a series of studies focusing on the ablation size (Section \ref{sec:ablation_size}), strided ablations (Section \ref{sec:ablation_stride}), and ablation type (Section \ref{sec:ablation_type}) in the ImageNet setting. 
% Notably, many of these studies are computationally infeasible for a CNN due to the scale of ImageNet, and are only practical when using a ViT to speed up training and inference as discussed previously in Section \ref{sec:speedup}. 

% \subsection{Ablation Size}
% We first study how the size of ablation (at both training and test time) affects certified performance. 
% In section~\ref{sec:ablation_size}, we saw that base classifiers can more accurately classify larger ablation sizes, but how does this affect certified robustness? After all, larger ablation sizes directly increases the necessary threshold for certification. In this section, we find that certified performance is largely stable with respect to ablation size, allowing allowing for a trade-off between computation time and clean accuracy without losing certified performance. 


% \begin{figure}[!htbp]
%     \centering
%         % \includegraphics[width=.48\textwidth]{figures/pretrained/imagenet_cert_acc.pdf}
%         % \includegraphics[width=.48\textwidth]{figures/pretrained/imagenet_smooth_acc.pdf}
%         \caption{Effect of ablation size at evaluation for column smoothed ImageNet models with columns of width $19$.}
%     \label{fig:ablation-size-eval}
% \end{figure}

% \paragraph{Ablation size for certification}
% As a first experiment, take various ViTs and ResNets trained on ImageNet column ablations of width $19$, and measure certified performance with respect to multiple ablation sizes in Figure \ref{ablation-size-eval}. 
% We find that certified accuracy is relatively stable over ablation sizes, peaking between column widths of 20-30px for all models.\footnote{The stability of certified accuracy to ablation size was previously observed by \citet{levine2020randomized} in the CIFAR10 setting, and we confirm that this is indeed holds in the more complex ImageNet setting.}
% However, clean accuracy makes significant gains with larger ablation sizes---improving ImageNet accuracy by almost 4\%  at column width $s=37$ with the same certified accuracy for the ViT-B model, while increasing inference time by TODO. 
% Consequently, varying the ablation size can lead to almost free improvements to clean accuracy. 
% %Here we show the effect of varying the ablation size for certifying pretrained ViTs and ResNets as shown in Figure~\ref{fig:ablation-size-pretrained}. These are complementary to the results of Section~\ref{sec:ablation_size}. 


% \begin{figure}[!htbp]
%     \centering
%         % \includegraphics[width=.48\textwidth]{figures/pretrained/imagenet_cert_acc.pdf}
%         % \includegraphics[width=.48\textwidth]{figures/pretrained/imagenet_smooth_acc.pdf}
%         \caption{Effect of ablation size at evaluation for column smoothed ImageNet models with columns of width $19$.}
%     \label{fig:ablation-size-train}
% \end{figure}

% \paragraph{Ablation size during training}
% In addition to certification time, we also explore varying ablation size seen at training time. 
% Specifically, we train train and certify a ResNet50 and ViT-S at the same ablation size over a range of column widths from 1 to 37px. 
% First, we find that once columns are wide enough, we see only marginal improvements in certified accuracy (i.e. only TODO\% over $s=19$). 
% This suggests that small ablations are sufficient at training time, allowing for fast training of ViTs when using cropped ablations. 
% Second, we see that ResNets require a substantially larger column width ($s=TODO$) in order to reach optimal certified accuracy---but still remains behind the ViT. 

% Overall, we find that certified performance on ImageNet remains largely stable with respect to column ablation size, allowing for faster training and improved clean accuracy. 

% % \begin{figure}[!htbp]
% %     \centering
% %     \begin{subfigure}[b]{.8\textwidth}
% %     \centering
% %         \includegraphics[width=.48\textwidth]{figures/pretrained/cifar10_cert_acc.pdf}
% %         \includegraphics[width=.48\textwidth]{figures/pretrained/cifar10_smooth_acc.pdf}
% %         \caption{Pretrained CIFAR-10 models.}
% %     \end{subfigure}
% %     \begin{subfigure}[b]{.8\textwidth}
% %         \centering
% %             \includegraphics[width=.48\textwidth]{figures/pretrained/imagenet_cert_acc.pdf}
% %             \includegraphics[width=.48\textwidth]{figures/pretrained/imagenet_smooth_acc.pdf}
% %             \caption{Pretrained ImageNet models.}
% %         \end{subfigure}
% %     \caption{Certified and clean accuracies of various \textbf{pretrained} DeiT and comparable size ResNet models on CIFAR-10 and ImageNet. DeiTs outperforms ResNets by a significant margin especially no ImageNet while maintaining competitive clean accuracies with standard trained SOTA models.}
% %     \label{fig:ablation-size-pretrained}
% % \end{figure}

% \subsection{Strided ablations}
% In order to speed up inference, one possibility is to use strided ablations to reduce the number of ablations. 
% Instead of using every possible column ablation, we can instead take every $s$th column ablation for a given stride $s$. An adversarial patch can intersect with a proportionally lower number of strided ablations, keeping the relative threshold for certification unchanged. 

% \begin{example}
% For column smoothing with width $b$ and stride $s$, the maximum number of ablations that an $m \times m$ patch can intersect with is at most $\Delta_{column+stride} = \lceil(m+s-1)/s\rceil$. 

% For block smoothing with block size $b$ and stride $s$, the maximum number of ablations that an $m \times m$ patch can intersect with is at most $\Delta_{block+stride} = \lceil(m+s-1)/s\rceil^2$. 
% \end{example}


% Using strided ablations reduces the total number of ablations (and consequently speeds up inference) by a factor of $s$, without substantially changing the threshold (up to rounding). 

% \subsection{Block smoothing}
% In this section, we consider block smoothing as an alternative to column smoothing in the ImageNet setting. 
% Note that a forward pass with block smoothing on ImageNet requires taking a majority vote over $224\times 224 = 50,176$ total ablations, which is extremely expensive. 
% Consequently, block smoothing for ImageNet is only reasonably computationally feasible when using the ViT with cropped ablations, which reduces runtime by about an order of magnitude. 

==> sections/studies.tex <==
In the previous section, we established that ViTs lead to  both more accurate and \textit{faster} certification than CNNs. 
% The speed up in certification that we get allow us to investigate in more detail various aspects of derandomized smoothing on large-scale datasets such as ImageNet. 
% In this section, we study the trade-offs between various aspects of derandomized smoothing: ablation size, ablation strides, and block vs. column smoothing.
However, specific choices in image ablation such as the type, amount, and size can significantly affect trade-offs between certified robustness and other metrics such as clean accuracy and inference speed. 
In this section, we demonstrate how these choices affect the smoothed model and the corresponding trade-offs through a series of studies focusing on the ablation size (Section \ref{sec:ablation_size}) and strided ablations (Section \ref{sec:ablation_stride}). 
Analogous experiments for the block smoothing instead of column smoothing are deferred to Appendix \ref{app:block-smoothing}---note that many of the block smoothing settings are computationally infeasible for a CNN in the ImageNet setting, and are only practical when using a ViT to speed up training and inference as discussed previously in Section \ref{sec:speed}. %\eric{Rewrite to reflect moving block smoothing to the appendix.}


\subsection{Ablation size}
\label{sec:ablation_size}
Derandomized smoothing certificates depends on the size of the unmasked part of the image, which we refer to as the \textit{ablation size}. 
For column smoothing for instance, this is the width of the column of pixels that remain unmasked in the ablation process. 
Previously in section~\ref{sec:ablations}, we saw that base classifiers can more accurately classify larger ablation sizes, but how does this affect certified robustness? 
After all, larger ablations directly increase the necessary threshold for certification and reduce certified performance. In this section, we find that certified performance is largely stable with respect to ablation size, allowing allowing for a trade-off between computation time and clean accuracy without losing certified performance. 
%Intuitively, as the ablation size changes, there is a trade-off between the certified accuracy and the clean accuracy; larger ablation sizes can increase the clean accuracy of the smooth classifier as it is seeing more of the images, but the fraction of ablations which intersects with a petential adversarial patche also increases, which might lead to decreases certified accuracy. So it is important to carefully choose what ablation size to use for derandomized smoothing.




\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{.8\textwidth}
    \centering
        \includegraphics[width=.48\textwidth]{figures/Finetuned/cifar10_cert_acc.pdf}
        \includegraphics[width=.48\textwidth]{figures/Finetuned/cifar10_smooth_acc.pdf}
        \caption{CIFAR-10 models.}
    \end{subfigure}
    \begin{subfigure}[b]{.8\textwidth}
        \centering
            \includegraphics[width=.48\textwidth]{figures/Finetuned/imagenet_cert_acc.pdf}
            \includegraphics[width=.48\textwidth]{figures/Finetuned/imagenet_smooth_acc.pdf}
            \caption{ImageNet models.}
        \end{subfigure}
    \caption{
    Certified and standard accuracy for a smoothed model trained on column ablations with width $b=19$, and evaluated with column ablations of varying width. Certified accuracy remains stable across a range of ablation sizes, while clean accuracy can substantially improve with larger ablations. 
    % \textbf{Test-time ablation size analsysis:} Certified and clean accuracies of various \textbf{finetuned} DeiTs and comparable size ResNet models on CIFAR-10 and ImageNet. DeiTs outperforms ResNets by a significant margin especially no ImageNet while maintaining competitive clean accuracies with standard trained SOTA models. \ericinline{we need to fix this caption, it has nothing to do with the section.}
    }
    \label{fig:ablation-size-finetuned}
\end{figure}

\paragraph{Test-time ablation}
As a first experiment, we study how ablation size effects certified and clean accuracy at test time. 
We consider the column smoothed models from Section \ref{sec:improve}. 
However, instead of certifying at column width $b=19$ (the ablation size used during training), we experiment with a range of ablations and report the clean and certified accuracy in Figure~\ref{fig:ablation-size-finetuned}. 

We find that certified accuracy is relatively stable over ablation sizes. For example, on ImageNet, certified performance peaks between column widths of 20-30px for all models.
% \footnote{\citet{levine2020randomized} previously observed the stability of certified accuracy to ablation size in the CIFAR10 setting. We replicate this finding and confirm that the same holds for the more complex ImageNet setting.}
However, clean accuracy makes significant gains with larger ablation sizes---improving ImageNet accuracy by almost 4\%  at column width $s=37$ with the same certified accuracy for the ViT-B model. 
Although the larger ablation size increases inference time for the ViT by a factor of TODO, this is still TODOx faster than the ResNet.\eric{saachi can you fill these in?}
Consequently, varying the ablation size can lead to almost free improvements to clean accuracy. 

%We study the effect of varying the ablation size at test time. We focus on the finetuning setting of derandomized smoothing, where the base models are trained with ablation, as shown in Figure~\ref{fig:ablation-size-finetuned}. As the ablation size increases, the smooth accuracies of all models increase as expected, but the certified accuracy increase then start decreasing after some ablation size for each model or dataset. For example on CIFAR-10, ViT-B obtains the highest certified accuracy of $65\%$ at an ablation size of $5$, afterwhich this accuracy starts droping (while the clean smooth accuracy continue increasing.). This also happens for ImageNet, but in a less severe manner. Thus it is really important to choose the ablation size appropriately when applying randomized smoothing in practice. Otherwise you might end up with a very high smooth accuracy but low certified accuracy.

% Similar results hold for the pretraining setting, but we defer these to Appendix~\ref{app:probing}). 

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{.48\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/training_ablation_sweep/ImageNet_cert_acc.pdf}
        % \caption{Finetuned CIFAR-10 models.}
    \end{subfigure}
    \begin{subfigure}[b]{.48\textwidth}
        \centering
            \includegraphics[width=\textwidth]{figures/training_ablation_sweep/ImageNet_smooth_acc.pdf}
            % \caption{Finetuned ImageNet models.}
        \end{subfigure}
    \caption{
    Certified and standard accuracy for a smoothed model trained and evaluated on ImageNet column ablations with varying widths. The ResNet50 requires a substantially larger ablation size for certification, whereas the ViT-S is more flexible. \ericinline{Hadi can you update this figure with the additional sizes?}
    %\textbf{Train-time ablation size analsysis:} Certified and clean accuracies of various \textbf{finetuned} DeiTs and comparable size ResNet models on CIFAR-10 and ImageNet. DeiTs outperforms ResNets by a significant margin especially no ImageNet while maintaining competitive clean accuracies with standard trained SOTA models. \ericinline{we need to fix this caption, it has nothing to do with the section.}
    }
    \label{fig:ablation-size-train-time}
\end{figure}

\paragraph{Train-time ablation}
In addition to certification time, we also explore varying the ablation size used at training time. 
Specifically, we train train and certify a ResNet-50 and ViT-S at the same ablation size over a range of column widths from 1 to 37px. 
First, we find that once columns are wide enough, we see only marginal improvements in certified accuracy (i.e. only TODO\% over $s=19$). 
This suggests that small ablations are sufficient at training time, allowing for fast training of ViTs when using cropped ablations. 
Second, we see that ResNets require a substantially larger column width ($s=TODO$) in order to reach optimal certified accuracy---but still remains behind the ViT. 

Overall, we find that certified performance on ImageNet remains largely stable with respect to column ablation size, allowing for faster training trains and trade-offs between speed and clean accuracy. 



\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{.48\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/stride_sweep/ImageNet_cert_acc.pdf}
        % \caption{Pretrained CIFAR-10 models.}
    \end{subfigure}
    \begin{subfigure}[b]{.48\textwidth}
        \centering
            \includegraphics[width=\textwidth]{figures/stride_sweep/ImageNet_smooth_acc.pdf}
            % \caption{Pretrained ImageNet models.}
        \end{subfigure}
    \caption{Certified accuracy of various ViTs and comparable size ResNets on CIFAR-10 and ImageNet. ViTs non-trivial robustness wheras ResNets do not.}
    \label{fig:stride-sweep}
\end{figure}


\subsection{Ablation strides}
\label{sec:ablation_stride}
The bulk of the runtime of derandomized smoothing comes from aggregating predictions over a large number of ablations. 
For example, column smoothing on ImageNet aggregates the result over $224$ column ablations, slowing down inference by two orders of magnitude. 
Although we previously sped this process up with cropped ablations for ViTs, another possibility is to use strided ablations to reduce the number of ablations. 
Specificaly, instead of using every possible ablation, we can instead take every $s$th ablation for a given stride $s$. 
Strided ablations reduces the total number of ablations (and consequently speeds up inference) by a factor of $s$, without substantially changing the certification threshold (up to rounding). 
%Note that the relative threshold for certification stays relatively unchanged, since an adversarial patch can intersect with a proportionally lower number of strided ablations. 

% \eric{Need to move strided block smoothing to the appendix}
\begin{example}
For column smoothing with width $b$ and stride $s$, the maximum number of ablations that an $m \times m$ patch can intersect with is at most $\Delta_{column+stride} = \lceil(m+s-1)/s\rceil$. 
\end{example}

% Derandomized smoothing has so far been aggregating the results over all %enumerations of columns of specific size in order to do a smoothed prediction and calculate robustness certificates. For example. for a $224\times 224$ image, the aggreation happens over 224 column ablations. As discussed in Section~\ref{sec:speed}, this requires many forward passes through the model inorder to get one prediciton/certificate which lead to slow-downs compared to standard (non-smoothed) models. 
%And although ViTs are able to accelerate this certification by utilizating its token-based nature, it would be great if we can speed things up even more. It turns out that we can subsample the set of ablations but doing strided ablations and still get really high certificates while getting 5-10x speedup in certification. Formally, if we use a stride length of $\gamma$ for our ablations (i.e., consider overlapping columns whose left corners are separated by $\gamma$ pixels), we directly get a speedup by a factor of $\gamma$. 

We test this for various ViTs on ImageNet, with column ablations of width $19$, against $32\times 32$ patches. 
We find multiple strides that achieve similar performance to the stride of length 1 (e.g. stride of 5 or 10) as shown in Figure~\ref{fig:stride-sweep}. 
These results comes at 5x and 10x speedups respectively, with slightly lower clean accuracy as shown in the right plot of Figure~\ref{fig:stride-sweep}. 
\eric{Hadi, can you help replace the right plot with a column smoothing equivalent? And move the current block smoothing one to the appendix?}
We find that striding can lead to high variance in performance: certified and standard accuracy can drastically shift either upwards or downwards as we vary the stride. 
% \eric{we should probably say something about the non-monotonic nature of the certified accuracy}
However, as long as the stride is carefully selected, we can trade-off a slight decreases in certified and clean accuracy for significant speedups in certification. 
\eric{Saachi, how close is this to a standard forward pass of a non-smoothed model?}


% \paragraph{Background on block smoothing}

% \paragraph{Experiment}
% We run a set of experiments on various ViTs, ablation sizes, and strides. The results are shown in Figure~\ref{}.

==> sections/why-transformers.tex <==
While certified methods such as derandomized smoothing can offer appealing robustness guarantees, they suffer steep degradations in accuracy and high computational costs. 
In this section, we quantitatively evaluate two properties of transformers that can alleviate these drawbacks. 
First, ViTs significantly outperform ResNets when given only a small column or patch of an image, and are thus better suited at processing image ablations (Section \ref{sec:ablations}). 
Second, since transformers operate on tokens, ViTs can drop masked-out portions of the image to greatly reduce the computational cost of derandomized smoothing (Section \ref{sec:speed}). 
%We then leverage the \textit{token-centric} approach of transformers, to lower the computational cost of evaluating image ablations by dropping the masked-out portions of the image (Section \ref{sec:speed}).  

% We now quantitatively evaluate to what extent transformers are better suited for processing image ablations than typical convolutional architectures such as ResNets. We demonstrate that: 
% \begin{enumerate}
%     \item ViTs are better than ResNets at classifying image ablations used in derandomized smoothing (Section \ref{sec:ablations}). 
%     % \item Unlike ResNets, pretrained ViTs can already provide non-trivial certificiates of patch robustness without ever having trained on image ablations (Section \ref{sec:pretrained}).
%     \item ViTs can drop masked-out patches to drastically accelerate inference of image ablations (Section \ref{sec:speed}). 
% \end{enumerate}
\paragraph{Setup:} %Our setup closely replicates that of \citet{levine2020randomized}. 
% We consider the setting of column-smoothing on the CIFAR10\citep{} and ImageNet \citep{} datasets. 
% We follow the same setup as specified by \citet{levine2020randomized}, by pre-training our base models on the standard dataset. 
%We use pretrained ResNets and ViT architectures and fine-tune them on randomly ablated images for a fixed column width. 
%Unless otherwise specified, we use the default parameters from \citep{levine2020randomized} (i.e. column width )
% for each image $x$ we draw a random $x' \sim S_{b_t}(x)$. Following \cite{leavitt2020towards}, we choose $b_t = 4$ for CIFAR10 and $b_t=19$ for ImageNet.
We consider the CIFAR-10~\citep{krizhevsky2009learning} and ImageNet~\citep{deng2009imagenet} datasets, and perform our analysis on three sizes of vision transformers---ViT-Tiny (Vit-T), ViT-Small (Vit-S), and ViT-Base (Vit-B) models \citep{rw2019timm, dosovitskiy2020image}. 
We compare to residual networks of \textit{similar size}---ResNet-18, ResNet-50 \citep{he2016deep}, and Wide ResNet-101-2 \citep{zagoruyko2016wide}, respectively.\footnote{Wide ResNet-101-2 is slightly larger than Vit-B.}. 
Further details about our experimental setup can be found in Appendix \ref{app:setup}. 
In this section, we study the patch certification setting considered in prior work \citep{levine2020randomized}: training with column ablations of size $b=4/32$ for CIFAR-10 and $b=19/224$ for ImageNet\footnote{Note that for ImageNet, \citet{levine2020randomized} use $s=25$ since they resize the images to 299x299, where as we use 224x224.}, and certifying robustness against $5\times 5$ patches for CIFAR10 and $32\times 32$ for ImageNet. 
%In section \ref{sec:why}, we quantitatively evaluate how much better transformers are at classifying image ablations and 

% \subsection{Barriers to Deploying Certified Models}
% [Eric] general note here: speed and accuracy not really things we identify as barriers for certified robustness, it's pretty well known
% While certified methods such as derandomized smoothing offer appealing robustness guarantees, they're not often deployed in practice. We identify two key barriers for practically deploying derandomized smoothing: \textit{accuracy and speed}. 

% \eric{This prelude can be greatly shortened and merged into the later sections, we also probably don't want this many numbers in the introduction to a section}


% [Eric] moving parts of these paragraphs down below instead
% \paragraph{Accuracy:} De-randomized smoothing requires the base classifier to accurately label an image even when given only a small column or patch. However, while a ResNet50 can achieve an accuracy of \saachiinline{X\%} on ImageNet, its accuracy drops to an average \saachiinline{X\%} when the model is only given \saachiinline{X\%}-wide columns of the image. Even if the ResNet has been fine-tuned to expect such ablations, the average ablation accuracy is \saachiinline{X\%}. This causes a large gap in performance between a regular ResNet and the smoothed classifier \saachiinline{X\%}, which can make deploying certifiably patch robust ResNets unfeasible.

% \paragraph{Speed:} Beyond accuracy, however, smoothing methods require $N$ inference runs of the base classifier, where $N$ is the number of ablations. For column smoothing on a 224x224 image, for example, certification would require $N$ forward passes of the base classifier. While these forward passes can be performed in parallel, randomized smoothing substantially increases the number of flops needed for inference, posing significant issues for tasks that require on-device inference with strict timing requirements, such as autonomous driving. 

% In this section, we show that Vision transformers can significantly improve over CNNs both in terms of accuracy on ablations and speed, and can thus ameliorate the deployment barriers that are faced by smoothed CNNs.

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/finetuned/cifar10_ablation_acc.pdf}
        \caption{CIFAR-10 models.}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/finetuned/ImageNet_ablation_acc.pdf}
        \caption{ImageNet models.}
    \end{subfigure}
\caption{Ablation accuracies for models on CIFAR-10 and ImageNet column-ablated images. The models were fine-tuned on column ablations of width $b=19/224$ for ImageNet and $b=4/32$ for CIFAR-10, and evaluated on a range of ablation sizes. ViTs outperform ResNets on image ablations by a sizeable margin.}
\label{fig:finetuned}
\end{figure}


\subsection{ViTs improve ablation accuracy}
\label{sec:ablations}
% \eric{is there a good name for these two properties?}
\eric{Consider moving CIFAR10 to appendix, for space}

The success of de-randomized smoothing methods hinges entirely on whether the base classifier can accurately classify subregions of an image, such as a small column or a patch. 
We thus measure the accuracy of fine-tuned ViTs for classifying column ablated images in comparison to ResNets across a range of evaluation ablation sizes \saachi{is it clear here that the training ablation size is not the same as the evaluation ablation size?}.

We find that ViTs are significantly more accurate on column ablations than comparably sized ResNets (Figure \ref{fig:finetuned}). 
This difference is most prominent on Imagenet---ViT-S has 11-12\% higher ablation accuracy across a range of ablation sizes than the the comparably sized ResNet-50. This suggests that ViTs are better suited for classifying image ablations. 

Since ViTs are substantially more accurate at processing image ablations than ResNets, we would expect them to also produce better certied defenses against patch attacks. 
In Section \ref{sec:improve}, we show how Smoothed ViTs have better accuracy and guarantees than Smoothed ResNets. 
\eric{need to revise this last two sentences}

%\paragraph{Pretrained} 

%These results suggest that the ViT architecture is naturally more robust to extreme masking of inputs than ResNets. 
%We find that pretrained ResNets have severely degraded ablation accuracy unlike pretrained ViTs, as shown in Figure \ref{fig:pretrained}. For example, a typical ResNet-50 pretrained on ImageNet classifies less than $5\%$ of column ablations correctly. In contrast, a pretrained Vit-S has a similar number of parameters but can correctly classify over $35\%$ of ablations. 
%\paragraph{Finetuned} 

%Base classifiers used for smoothing are typically fine-tuned to perform better on image ablations. We find that although the ResNet improves when fine-tuned, it is still not as good as the ViT at classifying ablations as shown in Figure \ref{fig:finetuned}. 
%\saachi{are we sure we want these to be paragraph tags? feels kind of like a bullet point list.}


% In Figure \ref{fig:pretrained}, we measure the ability of CNNs and ViTs pretrained on CIFAR-10 and ImageNet to predict the label of ablated images. Particularly on ImageNet, ViTs outperform CNNs by a substantial margin on ablation accuracy: on column-width of 25 pixels, for example, the ResNet-50 can correctly classify less than $5\%$ of ablations while a comparably sized Vit-small can correctly classify over $35\%$ of ablations.  \saachi{Do we want to put the smoothed performance here.} This suggests that ViTs are able to naturally handle patches or ablated data more gracefully than CNNS. This is arguably tied to the fact that vision transformers operate on image patch tokens, so are able to redirect attention to the non-masked portions of an ablted image. \saachi{We can't really support this sentence}

% \begin{figure}[!htbp]
%     % \centering
%     % \begin{subfigure}[b]{0.48\textwidth}
%     % \centering
%     %     % \includegraphics[width=\textwidth]{figures/pretrained/cifar10_ablation_acc.pdf}
%     %     \caption{Finetuned CIFAR-10 models.}
%     % \end{subfigure}
%     % \begin{subfigure}[b]{0.48\textwidth}
%     %     \centering
%     %     % \includegraphics[width=\textwidth]{figures/pretrained/ImageNet_ablation_acc.pdf}
%     %     \caption{Finetuned ImageNet models.}
%     % \end{subfigure}
% \caption{Dropping masked patches from ViTs does not harm performance.}
% \label{fig:missingness}
% \end{figure}


% \eric{replace this figure with ablation accuracy instead of certified accuracy, and move this to the appendix (they show similar things but ablation accuracy fits better here)}

\begin{table}
\begin{center}
\caption{We measure the average speed (over 50 trials) of computing a forward pass with a vision transformer on 1024 column ablated images with varying ablation sizes. We report the multiplicative speed up dropping masked tokens versus passing the full input to the  vision transformer.}
\label{tab:speed}
\begin{tabular}{c|cccccccccc}
\toprule
Ablation Size (px) & 13 & 19 & 25 & 31 & 37 & 43 & 49 & 55 & 61 & 67\\
\midrule
VIT-T & 10.62x & 6.44x & 6.44x & 4.33x & 3.48x & 3.48x & 3.48x & 2.91x & 2.90x & 2.90x\\
VIT-S & 10.57x & 6.40x & 4.39x & 4.40x & 4.41x & 3.52x & 3.52x & 3.52x & 2.93x & 2.93x\\
VIT-B & 11.63x & 6.76x & 6.75x & 4.51x & 3.62x & 4.50x & 3.63x & 3.61x & 2.94x & 2.94x\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

\subsection{ViTs reduce computational complexity}
\label{sec:speed}
% \eric{added an introductory section here as well, likely needs to be revised}
A downside of derandomized smoothing is its computational cost---a forward pass through the smoothed model requires passing all possible ablations through the base classifier. 
For column smoothing (the fastest type of ablation for derandomized smoothing) on a $s \times s$ pixel image, this is $s$ times slower than a normal forward pass. 
For ImageNet, this slows down evaluation by two orders of magnitude.
\eric{Fix notation}

% One possible approach to reduce this computation would be to pass only unmasked region of the image to the base classifier, effectively reducing the size of the input. However, for convolutional architectures, this restricts the ablation to be contiguous and strips all positional information from the input, leading to fewer ablations and reduced performance (see Appendix \ref{app:crop}). 

% [Eric] - it is not just certification, it is also for normal predictions. I think this is repeating the first paragraph so I commented this out for now
%During certification, the base classifier spends a significant amount of time processing the masked portions of the image. 
One natural strategy for reducing unnecessary computation is to crop out the masked regions before passing the image to the base classifier. Although reducing the size of the image can speed up inference, cropping has several downsides for CNNs. Cropping an image strips spatial information about the ablation and disallows ablations that wrap around the sides of the image. These lead to substantial reductions in certified performance which we discuss in more detail in Appendix \ref{app:crop}. 
%One possible strategy for reducing unnecessary computation would be to crop out the masked regions before passing the image to the base classifier. However, this approach would strip spatial information about where the unmasked region is located in the image. Moreover, since convolutional architectures only accept contiguous inputs, this optimization would disallow ablations that wrap around the sides of the image. In Appendix \ref{app:crop}, we find that cropping leads to significantly reduced performance.  

%While passing a cropped version of the image could avoid some of this computation, it would restrict ablations to be contiguous and would strip all positional information from the input. 

% \eric{this is going to be super confusing to people that aren't familiar with transformers, we definitely need a graphic here}
% However, unlike CNNs, Vision Transformers are inherently a \textit{token-based} model. Beyond an initial positional encoding stage, each self-attenton layer processes an unordered set of tokens, expressing each token as a linear combination of the other tokens. For smoothing, we can
% positionally encode \textit{only the unablated} tokens with their position 
% in the original image, and then pass only those tokens through the transformer.
% The transformer thus processes only the unablated tokens while retaining 
% all positional information. 

However, unlike CNNs which require a structured input, Vision Transformers operate on \textit{tokens}, where each token corresponds to a region in the image. 
Crucially, transformers treat inputs as unordered sets of tokens, which can be of any size and do not have to be contiguous in the original image space. 
Thus, we can perform the following simple procedure to avoid computation on fully masked tokens:
\begin{enumerate}
    \item Positionally encode the entire ablated image into tokens\;
    \item Drop any tokens that correspond to a fully masked region of the image\;
    \item Pass the remaining tokens through the transformer\;
\end{enumerate}
A more detailed discussion of this optimization can be found in Appendix \ref{app:droptokens}



%Thus, during smoothing, we can simply pass a \textit{subset} of the tokens to the transformer, dropping any tokens which correspond to fully masked regions of the image. 

\paragraph{Performance impact}
Since the tokens are encoded with their spatial location in the original input, we do not lose any positional information when dropping tokens. 
In practice, we find that dropping masked tokens does not hurt performance as shown in Figure \ref{fig:missingness-ablation-acc}. 
Dropping tokens thus amounts to a free speed-up for ViTs, reducing runtime as shown in Table \ref{tab:speed}. 
%In contrast to convolutional architectures, ignoring masked patches for the transformer does not hurt performance as shown in Figure \ref{fig:missingness-ablation-acc}. 
% Table \ref{tab:speed} shows the empirical speedup we get from dropping masked patches. 
% \eric{I think the missingness plot that shows no performance drop goes very nicely here}


\paragraph{Computational Complexity} 
%Most of the image is masked during smoothing, this optimization can significantly reduce computation costs. 
\eric{Fix notation}
More formally, suppose the base classifier is a ViT that takes a $s \times s$ pixel image embeds patches of $p \times p$ into tokens. 
Processing the full image thus requires evaluating $O(s^2/p^2)$ tokens with the ViT. 
To process a column ablation with width $b$, we can drop masked tokens and only evaluate $O(bs/p^2)$ tokens with the ViT, reducing the number of tokens by a factor of $O(s/b)$. 

It turns out that passing fewer tokens can drastically speed up certification beyond an $O(s/b)$ factor. 
Specifically, the self-attention mechanism of the ViT scales quadratically with the number of tokens. 
Thus, the complexity for evaluating a full image is $O(s^4/p^4)$, which reduces to $O(b^2s^2/p^4)$ when dropping masked tokens for column ablation. 
In fact, the cost of inference for a smoothed ViT with dropped tokens is almost comparable to a forward pass for a standard ViT. 
For example, column smoothing evaluates $s$ different ablations, incurring a total runtime cost of $O(b^2s^3/p^4)$. 
For $b \leq \sqrt{s}$, a smoothed ViT can actually be faster than a standard ViT. 
%In fact, for $b \leq \sqrt{s}$, computing the smoothed classifier is actually faster than a single forward pass on a full-sized image.
\eric{this section is kind of chunky}
\eric{Reference analogous results for block smoothing in the appendix}


\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/finetuned_missingness/cifar10_ablation_acc.pdf}
        \caption{CIFAR-10 models.}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/finetuned_missingness/imagenet_ablation_acc.pdf}
        \caption{ImageNet models.}
    \end{subfigure}
\caption{Ablation accuracies for various Vit models on CIFAR-10 and ImageNet, with and without missingness. The performance of both are comparable to each other while the missigness ones are 2 orders of magnitude faster.\ericinline{Fix this caption; also is 2 order of magnitude correct??}}
\label{fig:missingness-ablation-acc}
\end{figure}



% Since each self-attention layer scales quadratically with the number of tokens, this optimization can dramatically speed up the certification process. For smaller ablations, certification can actually be faster than a single forward pass on the full image. Suppose the base classifier is a transformer that takes a $c \times c$ pixel image and embeds $p \times p$ patches into tokens. The transformer when evaluating a full image will process $c^2/p^2$ tokens, for an overall runtime of $O(c^4/p^4)$. However, for band smoothing with a width of $b$, the base classifier will perform $c$ passes with $bc/p^2$ tokens, resulting in a runtime of $O(b^2c^3/p^4)$. Thus, for $b \leq \sqrt{c}$, full certification via de-randomized smoothing is faster than a single forward pass on a full-sized image. \saachi{insert scalability examples here}

